Testing Uniform Random Samplers: Methods, Datasets and Protocols

Boolean formulae compactly encode huge, constrained search spaces. Thus, variability-intensive systems are often encoded with Boolean formulae. The search space of a variability-intensive system is usually too large to explore without statistical inference (e.g. testing). Testing every valid configuration is computationally expensive (if not impossible) for most systems. This leads most testing approaches to sample a few configurations before analyzing them. A desirable property of such samples is uniformity: Each solution should have the same selection probability. Uniformity is the property that facilitates statistical inference. This property motivated the design of uniform random samplers, relying on SAT solvers and counters and achieving different trade-offs between uniformity and scalability. Though we can observe their performance in practice, judging the quality of the generated samples is different. Assessing the uniformity of a sampler is similar in nature to assessing the uniformity of a pseudo-random number (PRNG) generator. However, sampling is much slower and the nature of sampling also implies that the hyperspace containing the samples is constrained. This means that testing PRNGs is subject to fewer constraints than testing samplers. We propose a framework that contains five statistical tests which are suited to test uniform random samplers. Moreover, we demonstrate their use by testing seven samplers. Finally, we demonstrate the influence of the Boolean formula given as input to the samplers under test on the test results.

==> parts/9-Data_availability.tex <==
We provided our replication package in the form of an anonymous Github: \url{} ...

To reproduce our experiments you must run the following commands ...

\ma{please indicate the the full command to reproduce RQ1}

==> parts/uniformity.tex <==
\begin{tabular}{m{7em}|c|c|c|c}
%\toprule
       Sampler & \#Tests &  \#U & \#NotU & \#NA \\
\midrule
Distance-based &    188 &  13 &   164 &  11 \\
           KUS &    103 &  82 &     7 &  14 \\
           STS &    194 &  22 &    37 & 135 \\
% CustomSampler &    193 & 172 &     0 &  21 \\
       UniGen3 &     98 &  58 &     0 &  40 \\
       UniGen2 &     97 &  54 &     0 &  43 \\
  QuickSampler &    194 &   0 &   178 &  16 \\
        UniGen &     57 &   0 &     0 &  57 \\
        SMARCH &    198 &   0 &   187 &  11 \\
%\bottomrule
\end{tabular}

